Life in a random universe: Sciama's argument reconsidered

Random sampling in high dimensions has successfully been applied to phenomena as diverse as nuclear resonances, neural networks and black hole evaporation. Here we revisit an elegant argument by the British physicist Dennis Sciama, which demonstrated that were our universe random, it would almost certainly have a negligible chance for life. Under plausible assumptions, we show that a random universe can masquerade as `intelligently designed,' with the fundamental constants instead appearing to be fined tuned to be achieve the highest probability for life to occur. For our universe, this mechanism may only require there to be around a dozen currently unknown fundamental constants. We speculate on broader applications for the mechanism we uncover.

==> paper.tex <==


project.

\appendix

\section{Projection of an $\MakeLowercase{(n-1)}$-sphere to one dimension}

Consider a smooth convex $n$-dimensional geometric body with a uniform
probability distribution across and within it. The projective central
limit theorem claims that as $n\to\infty$, if we project such a body to
lower dimensions, the probability will concentrate to a `center' of
the lower dimensional object \cite{Diaconis1984,Klartag2007,Knaeble2015Ap}.
This phenomenon has been proved for all smooth convex geometric bodies
and the limiting probability distribution is claimed to be a Gaussian
distribution with variance scaling as $1/n$.

Here we compute this exactly for an $(n-1)$-sphere (the surface of an
$n$-dimensional ball) projected to $m$ dimensions. We find for large
$n-m$ that the resulting distribution is Gaussian with variance scaling
as $1/n$. This is in agreement with the more general, though
looser claim of the projective central limit theorem when $n\gg m$.
Finally, combining the `orange peel' concentration of measure
result, we argue that the same limit to a Gaussian with variance scaling as
$1/n$ will hold for the projection of an $n$-dimensional ball onto
$m$ dimensions.

Because the general calculation is rather complicated, we start with
the simpler case of projecting an $(n-1)$-sphere onto a single dimension.

An $(n-1)$-sphere with unit radius in n-dimensional Euclidean space
(Cartesian coordinates) may be described as satisfying $x^2_1+x^2_2+\cdots
+x^2_n=1$. It may be transformed into the hyper-spherical coordinate by
\begin{eqnarray}
x_1 &=& -\cos \varphi_1 \nonumber \\
x_2 &=& -\sin \varphi_1 \cos \varphi_2 \nonumber \\
&\vdots & \nonumber \\
x_{n-1} &=& -\sin \varphi_1 \sin \varphi_2 \cdots \cos \varphi_{n-1}
\nonumber \\
x_n &=& -\sin \varphi_1 \sin \varphi_2 \cdots \sin \varphi_{n-1} ,
\label{coordinate}
\end{eqnarray}
where $\varphi_1, \varphi_2, \ldots, \varphi_{n-2} \in [ 0,\pi ]$ and
$\varphi_{n-1} \in [0,2\pi]$. Here the minus sign is just for future
convenience; note that each $x_i$ is not sensitive to such a minus sign.

Then in hyper-spherical coordinates, the volume element of such an
$(n-1)$-sphere may be written
\begin{equation}
d\Omega_{n-1} = \sin^{n-2} (\varphi_1) \sin^{n-3} (\varphi_2) \cdots
 \sin^2 (\varphi_{n-3})  \sin (\varphi_{n-2}) \, d\varphi_1 d\varphi_2
 \cdots d \varphi_{n-2} d\varphi_{n-1} ,
\label{nsphere}
\end{equation}
as is easily checked by computing the Jacobian for this transformation.
Integrating this volume element over the entire sphere yields the
standard result
\begin{eqnarray}
S_{n-1} &=&\int d\Omega_{n-1} \nonumber \\
    &=& \int\sin^{n-2} (\varphi_1) \sin^{n-3} (\varphi_2)
 \cdots  \sin^2 (\varphi_{n-3})  \sin (\varphi_{n-2})
 \, d\varphi_1 d\varphi_2 \cdots d \varphi_{n-2} d\varphi_{n-1} \nonumber \\ 
    &=& \pi^{\frac{n-2}{2}} \frac{\Gamma(\frac{n-1}{2})}{\Gamma(\frac{n}{2})}
\frac{\Gamma(\frac{n-2}{2})}{\Gamma(\frac{n-1}{2})}
  \cdots  \frac{\Gamma(\frac{2}{2})}{\Gamma(\frac{3}{2})} 2\pi \nonumber \\ 
    &=& \frac{2 \pi^{\frac{n}{2}} }{\Gamma(\frac{n}{2})}  ,
\end{eqnarray}
where $\Gamma(n)$ is the gamma function so $\Gamma(1)=1$, and in
moving from the second to the third line we have used the result
that
\begin{equation}
\int_0^\pi
\sin^m(\varphi)\, d\varphi = \sqrt{\pi}\,
\frac{\Gamma(\frac{m+1}{2})}{\Gamma(\frac{m+2}{2})}.
\end{equation}

We now consider projecting the uniformly distributed $(n-1)$-sphere
onto a single dimension (i.e., the case $m=1$).
Normalizing the measure of Eq.~(\ref{nsphere}) by $S_{n-1}$, we may compute
the expectation of a general function of $\varphi_1$ as
\begin{eqnarray}
\langle f(\varphi_1)\rangle
&=&\frac{1}{S_{n-1}}\int f(\varphi_1) d\Omega_{n-1} \nonumber \\
    &=& \frac{1}{S_{n-1}} \int^\pi_0 f(\varphi_1) \sin^{n-2} (\varphi_1)
 \, \pi^{\frac{n-3}{2}}  \frac{\Gamma(\frac{n-2}{2})}{\Gamma(\frac{n-1}{2})}
  \frac{\Gamma(\frac{n-3}{2})}{\Gamma(\frac{n-2}{2})}
\cdots  \frac{\Gamma(\frac{2}{2})}{\Gamma(\frac{3}{2})}
2\pi \, d\varphi_1   \nonumber \\
    &=& \frac{\Gamma(\frac{n}{2}) }{2 \pi^{\frac{n}{2}}}
\int^\pi_0 f(\varphi_1) \sin^{n-2} (\varphi_1) \, 
 \frac{2 \pi^{\frac{n-1}{2}}}{\Gamma(\frac{n-1}{2})} \, d\varphi_1 
 \nonumber \\ 
    &=& \int^\pi_0 f(\varphi_1) \sin^{n-2} (\varphi_1) \, 
 \frac{ \Gamma(\frac{n}{2}) }{\sqrt{\pi}\, \Gamma(\frac{n-1}{2})}
\, d\varphi_1  .
\label{shpereP1}
\end{eqnarray}
Consequently, the distribution on $\varphi_1$ is given by
\begin{equation}
\text{P} (\varphi_1)\, d\varphi_1=
\sin^{n-2} (\varphi_1) \, 
 \frac{ \Gamma(\frac{n}{2}) }{\sqrt{\pi}\, \Gamma(\frac{n-1}{2})}
\, d\varphi_1 , \qquad \varphi_1\in [0,\pi]
\label{distP1}
\end{equation}
To see the probability distribution in Euclidean space, we need to
transform Eq.~(\ref{distP1}) back to the coordinate
$x_1$. Since $x_1=-\cos\varphi_1$, we have $dx_1=\sin \varphi_1
d\varphi_1$ and $\sin(\varphi_1)=\sqrt{1-x^2_1}$ and hence we obtain
\begin{equation}
\text{P} (x_1)\, dx_1=
\frac{ \Gamma(\frac{n}{2}) }{\sqrt{\pi}\,
\Gamma(\frac{n-1}{2})} (1-x_1^2)^{\frac{n-3}{2}} dx_1, \qquad x_1 \in [-1,1].
\label{shpereP3}
\end{equation}
We may also obtain an exact expression for the variance
\begin{equation}
(\Delta x_1)^2 = \frac{1}{n}.
\end{equation}

It is easy to see that this probability distribution gets narrower and
narrower as $n$ increases. Using the result that $\lim_{n \to \infty}
(1-\frac{x}{n})^n=e^{-x}$ we see that for sufficiently small $x_1$ and
large $n$ Eq.~(\ref{shpereP3}) may be approximated by a Gaussian with
variance $1/n$, for the case $m=1$. This result is in exact agreement
with that given in previous work \cite{Knaeble2015Ap}, we shall see below
that the exact result yields a subtly different outcome for $m>1$.

\section{Projecting to $\MakeLowercase{m}$-dimension}

When projecting an $(n-1)$-sphere onto $m$ Cartesian dimensions, the
logic is similar to that given in the previous section but now we will
need to integrate out the angles from the set $\{\varphi_{m+1},
\varphi_{m+2}, \ldots, \varphi_{n-1}\}$. Thus, we find
\begin{eqnarray}
\!\!\!&&\langle f(\varphi_1,\ldots,\varphi_m)\rangle
=\frac{1}{S_{n-1}}\int f(\varphi_1,\ldots,\varphi_m)\,d\Omega_{n-1} \nonumber \\
    &=& \frac{1}{S_{n-1}} \int^\pi_0 \cdots  \int^\pi_0
f(\varphi_1,\ldots,\varphi_m)\,
\sin^{n-2} (\varphi_1) \sin^{n-3} (\varphi_2)
\cdots \sin^{n-m-1} (\varphi_m) \nonumber \\
&&\phantom{\frac{1}{S_{n-1}} \int^\pi_0 \cdots  \int^\pi_0}
\times \pi^{\frac{n-m-2}{2}}
 \frac{\Gamma(\frac{n-m-1}{2})}{\Gamma(\frac{n-m}{2})}
 \frac{\Gamma(\frac{n-m-2}{2})}{\Gamma(\frac{n-m-1}{2})}
\cdots  \frac{\Gamma(\frac{2}{2})}{\Gamma(\frac{3}{2})}\,
2\pi \, d\varphi_1 d\varphi_2 \cdots d\varphi_m  \nonumber \\
    &=& \frac{\Gamma(\frac{n}{2}) }{2 \pi^{\frac{n}{2}}}
\int^\pi_0 \cdots  \int^\pi_0 f(\varphi_1,\ldots,\varphi_m)\,
\sin^{n-2} (\varphi_1) \sin^{n-3} (\varphi_2) \cdots \sin^{n-m-1}
(\varphi_m) \, \frac{2 \pi^{\frac{n-m}{2}}}{\Gamma(\frac{n-m}{2})}
\, d\varphi_1 d\varphi_2 \cdots d\varphi_m  \nonumber \\ 
    &=& \int^\pi_0 \cdots  \int^\pi_0 f(\varphi_1,\ldots,\varphi_m)
\sin^{n-2} (\varphi_1) \sin^{n-3} (\varphi_2) \cdots
\sin^{n-m-1} (\varphi_m) \,
  \frac{ \Gamma(\frac{n}{2}) }{\pi^{\frac{m}{2}}
\Gamma(\frac{n-m}{2})} \, d\varphi_1 d\varphi_2 \cdots d\varphi_m  .
\label{mshpereP1}
\end{eqnarray}
Since the volume element described by two different coordinates systems
may be connected by the Jacobian, we have 
\begin{equation}
dx_1 dx_2 \cdots dx_m = \text{J} \, d\varphi_1 d\varphi_2 \cdots d\varphi_m ,
\label{Ctransf1}
\end{equation}
where J is the Jacobian describes this volume transformation.
From Eq.~(\ref{coordinate}), we know that J may be written as
\begin{eqnarray}
\text{J} = \Bigl | \frac{\partial x_i}{\partial \varphi_j} \Bigr |  =
\left| \begin{array}{cccc}
\sin\varphi_1 & 0 & \cdots & 0 \\
\cos\varphi_1\cos\varphi_2 & \sin\varphi_1\sin\varphi_2 & \cdots & 0 \\
\vdots & \vdots & \ddots & \vdots \\
\cos\varphi_1\sin\varphi_2\cdots\sin\varphi_{m-1}\cos\varphi_m & \sin\varphi_1\cos\varphi_2\cdots\sin\varphi_{m-1}\cos\varphi_m & \cdots & \sin\varphi_1\cdots\sin\varphi_m
\end{array} \right|
\label{Jac1}
\end{eqnarray}
Since terms in the upper triangle in the Jacobian, Eq.~(\ref{Jac1}),
are all zero, the Jacobian trivially reduces to
\begin{eqnarray}
\text{J} = \sin ^m (\varphi_1) \sin ^{m-1} (\varphi_2)
\cdots \sin (\varphi_m) .
\label{Jac2}
\end{eqnarray}
Inserting Eq.~(\ref{Jac2}) into Eq.~(\ref{Ctransf1}) yields
\begin{equation}
dx_1 dx_2 \cdots dx_m = \sin ^m (\varphi_1) \sin ^{m-1} (\varphi_2)
\cdots \sin (\varphi_m) \, d\varphi_1 d\varphi_2 \cdots d\varphi_m ,
\label{Ctransf2}
\end{equation}
and substituting Eq.~(\ref{Ctransf2}) into Eq.~(\ref{mshpereP1}) yields
\begin{eqnarray}
&&\langle f(\varphi_1,\ldots,\varphi_m) \rangle \nonumber \\
&=&\int^1_{-1} \int_{-\sin \varphi_1}^{\sin \varphi_1}
\cdots  \int_{-\sin (\varphi_1) \cdots
\sin (\varphi_{m-1})}^{\sin (\varphi_1)
\cdots \sin (\varphi_{m-1})}f(\varphi_1,\ldots,\varphi_m)\,
 \sin^{n-m-2} (\varphi_1)
\sin^{n-m-2} (\varphi_2) \cdots \sin^{n-m-2} (\varphi_m) \nonumber \\
&&\phantom{\int^1_{-1} \int_{-\sin \varphi_1}^{\sin \varphi_1}
\cdots  \int_{-\sin (\varphi_1) \cdots
\sin (\varphi_{m-1})}^{\sin (\varphi_1)
\cdots \sin (\varphi_{m-1})} }
  \times \frac{ \Gamma(\frac{n}{2}) }{\pi^{\frac{m}{2}}
\Gamma(\frac{n-m}{2})} \, dx_1 dx_2 \cdots dx_m  , \nonumber \\
\label{mshpereP2}
\end{eqnarray}
where $\sin (\varphi_i)$ is positive function of $x_i$.

To further simplify Eq.~(\ref{mshpereP2}), let us first consider
$x^2_1 + x^2_2 + \cdots + x^2_m$. From Eq.~(\ref{coordinate}), this
may be written as
\begin{eqnarray}
x^2_1 + x^2_2 + \cdots + x^2_m 
&=& \cos^2 (\varphi_1) + \sin^2 (\varphi_1) \cos^2 (\varphi_2)
+ \cdots + \sin^2 (\varphi_1) \sin^2 (\varphi_2)
\cdots \cos^2 (\varphi_m) \nonumber \\ 
&=& \cos^2 (\varphi_1) + \sin^2 (\varphi_1) ( 1-\sin^2 (\varphi_2) )
+ \cdots + \sin^2 (\varphi_1) \sin^2 (\varphi_2)
\cdots \cos^2 (\varphi_m) \nonumber \\ 
&=& 1 - \sin^2 (\varphi_1) \sin^2 (\varphi_2)  + \cdots +
\sin^2 (\varphi_1) \sin^2 (\varphi_2) \cdots \cos^2 (\varphi_m) .
\end{eqnarray}
The above procedure can be repeated until we arrive at
\begin{eqnarray}
x^2_1 + x^2_2 + \cdots + x^2_m = 1 - \sin^2 (\varphi_1) \sin^2 (\varphi_2)
\cdots \sin^2 (\varphi_m) .
\label{x2x2}
\end{eqnarray}
Applying Eq.~(\ref{x2x2}) to Eq.~(\ref{mshpereP2}) then gives
\begin{eqnarray}
&& \langle f(x_1,\ldots,x_m)\rangle\nonumber \\
&=& \int^1_{-1} \int_{-\sqrt{1-x_1^2}}^{\sqrt{1-x_1^2}} \cdots 
\int_{-\sqrt{1-x_1^2-x_2^2-\cdots -x_{m-1}^2}}
^{\sqrt{1-x_1^2-x_2^2-\cdots -x_{m-1}^2}}
f(x_1,\ldots,x_m)\,
\frac{ \Gamma(\frac{n}{2}) }{\pi^{\frac{m}{2}}
f(x_1,\ldots,x_m)
\Gamma(\frac{n-m}{2})}  \Bigl( 1-\sum_{i=1}^{m} x_i^2
\Bigr)^{\frac{n-m-2}{2}} dx_1 dx_2 \cdots dx_m  , \nonumber \\
\label{mshpereP3}
\end{eqnarray}


By spherical symmetry, it is sufficient to compute the variance on $x_1$, but
this trivially reduces to the result already obtained, since to compute
it we may integrate out all the remaining coordinates $x_2,\ldots,x_m$.
Therefore we find exactly
\begin{eqnarray}
\langle x_i \rangle &=& 0 \nonumber \\
\langle x_i x_j \rangle &=& \delta_{ij} (\Delta x_i)^2 
=\frac{\delta_{ij}}{n}.
\end{eqnarray}
From similar reasoning, for sufficiently large $n$ the distribution 
becomes Gaussian.

Therefore, the probability distribution over this reduced m-sphere reduces
to
\begin{equation}
\text{P} (x_1, x_2, \cdots, x_m) =
\frac{ \Gamma(\frac{n}{2}) }{\pi^{\frac{m}{2}}
\Gamma(\frac{n-m}{2})} \,
\Bigl( 1-\sum_{i=1}^{m} x_i^2 \Bigr)^{\frac{n-m-2}{2}} ,
\end{equation}
with suitable limits on the $x_i$.
This is for the projection of an $(n-1)$-sphere to an $m$-dimensional
subspace.

The limit of this distribution as ${n-m} \to \infty$ and sufficiently
small $x_i$, $i\in\{1,\ldots,m\}$, may be approximated by a Gaussian
with mean zero and a variance in every direction of $1/n$. This result
agrees with previous work \cite{Knaeble2015Ap}, except on the condition
needed, here $n-m$ large as opposed to merely $n$ being large. The
difference in this requirement means that as $m\to n$, where we
project out fewer and fewer coordinates and finally none, the Gaussian
approximation is found to wholly fail.



\section{Projection of a rotated hypercube to two dimensions}

Our analysis, both analytic and numeric has largely been based on the
projection of high-dimensional hyperballs. Here we consider the
numerical projection of a randomly rotated high-dimensional hypercube to
two dimensions. Although computing the X-ray of such a hypercube is
straightforward, computing the projection of the boundary very quickly
becomes computationally inaccessible. In particular, one needs to take
the $2^n$ corners of the hypercube and project them to the lower
dimension of interest and then compute the convex hull of those
projected corners. This convex hull represents the `shadow' of the
rotated hypercube under ordinary light (which is assumed to be unable to
penetrate the object itself). In Fig.~\ref{fig4} we illustrate this
computation, comparing both the X-rays and shadows projected onto two
dimensions of (a) a 33-dimensional hyperball and (b) a randomly rotated
20-dimensional hypercube (the highest dimension we could compute in a
reasonable amount of time).

\begin{figure}[t]
\centering
% \vskip -0.1truein
\includegraphics[width=0.7\textwidth]{Fig4.pdf}
\vskip -0.1truein

\caption{Plots of both the X-ray (as a scatter plot of 2000
points) where a higher density of points represents a larger weight of
material being X-rayed and the `shadow' outline projection onto two
dimenstions of a (a) 33-dimensional hyperball and a (b) randomly
oriented 20-dimensional hypercube. For the shadow of the hypercube, the
dots along the outline represent the location of the corners there.}

\vskip -0.1truein
\label{fig4}
\end{figure}

As can be seen, in sufficiently high dimensnions the shadow of a
randomly rotated hypercube, Fig.~\ref{fig4}(b), looks remarkably like
that of a hyperball, Fig.~\ref{fig4}(a). Further, up to defining a
suitable `diameter' to make a more rigorous comparison, the X-ray
projection of such hypercubes appears remarkably similar to that of the
hyperball (again see Fig.~\ref{fig4}). Consequently, in our main
manuscript we used a hyperball to compute the threshold illustrated by
Fig.~3 there in even higher dimensions than we can manage for
hypercubes.

Were much larger computational facilities available a more careful
comparison should be possible, though even only a 42-dimensional
hypercube entails over 4 trillion corners, so computing the projected
boundary into any dimension greater than one \cite{Knaeble2015Ap}
would require major
computational effort.




\begin{thebibliography}{99}

\bibitem{Misner1970}
C.\ W.\ Misner, K.\ S.\ Thorne \& J.\ A.\ Wheeler,
{\it Gravitation},
(Freeman \& Co., San Francisco, 1973) p.~1216.

\bibitem{Weinberg1987}
S.\ Weinberg,
Anthropic bound on the cosmological constant
{\it Physical Review Letters\/} {\bf 59}, 2607-2610 (1987).

\bibitem{Weinberg1998}
H.\ Martel, P.\ R.\ Shapiro, S.\ Weinberg,
Likely values of the cosmological constant,
{\it The Astrophysical Journal}
{\bf 492}, 29-40 (1998).

\bibitem{Piran2016}
T.\ Piran, et al.,
Cosmic explosions, life in the universe, and the cosmological constant,
{\it Physical Review Letters\/} {\bf 116}, 081301 (2016).

\bibitem{Hoyle1954}
F.\ Hoyle, 
On nuclear reactions occurring in very hot stars. I.\ The synthesis of
elements from carbon to nickel,
{\it The Astrophysical Journal Supplement Series}
{\bf 1}, 121-146 (1954).

\bibitem{Carter1974}
B.\ Carter,
Large number coincidences and the anthropic principle in cosmology,
in {\it Confrontation of Cosmological Theories with Observational Data},
(Springer, Dordrecht, 1974) p.~291-298.

\bibitem{Adams2019}
Fred C.\ Adams,
The degree of fine-tuning in our universe -- and others,
{\it Physics Reports\/}
{\bf 807}, 1-111 (2019).

\bibitem{Dicke1961}
R.\ H.\ Dicke,
Dirac’s cosmology and Mach’s principle,
{\it Nature\/} {\bf 192}, 440-441 (1961).

\bibitem{Deutsch2011}
D.\ Deutsch, 
{\it The Beginning of Infinity: Explanations that Transform the World}
(Penguin, London, 2011), pp.~99-100.

\bibitem{Wang2023}
Z.-W.\ Wang, S.\ L.\ Braunstein,
Sciama’s argument on life in a random universe and
distinguishing apples from oranges,
{\it Nature Astronomy\/} {\bf 7}, 755-756 (2023).

\bibitem{Milman1988}
V.\ D.\ Milman, 
The heritage of P.\ L\'evy in geometrical functional analysis,
{\it Ast\'erisque} {\bf 157}, 273-301 (1988).

\bibitem{Eddington1936}
A.\ S.\ Eddington,
{\it Relativity Theory of Protons and Electrons}
(Cambridge Univ.\ Press, Cambridge, 1936) p.~3, 

\bibitem{Siegel2018}
E.\ Siegel,
How many fundamental constants does it take to explain the universe?
Forbes, Nov.\ 16, 2018.

\bibitem{Diaconis1984}
P.\ Diaconis \& D.\ Freedman, 
Asymptotics of graphical projection pursuit, 
{\it The Annals of Statistics}
{\bf 12}, 793-815 (1984).

\bibitem{Klartag2007}
B.\ Klartag, 
A central limit theorem for convex sets, 
{\it Inventiones Mathematicae} 
{\bf 168},  91-131 (2007).

\bibitem{Eddington1939}
A.\ S.\ Eddington,
{\it The Philosophy of Physical Science}
(Cambridge Univ.\ Press, Cambridge, 1939).

\bibitem{Cirkovic2016}
M.\ M.\ \'Cirkovi\'c,
Fermi’s Paradox Is a Daunting Problem -- Under Whatever Label,
{\it Astrobiology}, {\bf 16}, 737-740 (2016).

\bibitem{SETI}
D. Overbye,
The Search for E.T.\ Goes on Hold, for Now,
{\it The New York Times}, March 23, 2020.

\bibitem{Wilde1889}
O.\ Wilde,
The decay of lying: A dialogue,
in {\it The Nineteenth Century: A Monthly Review},
ed.\ J.\ Knowles. Vol. XXV. January-June, 1889. pp.~35-56. 


%\bibitem{Diaconis1984}
%P.\ Diaconis \& D.\ Freedman, 
%Asymptotics of graphical projection pursuit, 
%{\it The Annals of Statistics}
%{\bf 12}, 793-815 (1984).

\bibitem{Knaeble2015Ap}
B. Knaeble, 
Variations on the projective central limit theorem, 
{\it General Mathematics Notes\/}
{\bf 26(2)},  119-133 (2015).

%\bibitem{Klartag2007}
%B.\ Klartag, 
%A central limit theorem for convex sets, 
%{\it Inventiones Mathematicae} 
%{\bf 168},  91-131 (2007).

\end{thebibliography}




\end{document}



